Coordinated Multi-area Economic Dispatch via Critical Region Projection

A coordinated economic dispatch method for multi-area power systems is proposed. Choosing boundary phase angles as coupling variables, the proposed method exploits the structure of critical regions in local problems defined by active and inactive constraints. For a fixed boundary state given by the coordinator, local operators compute the coefficients of critical regions containing the boundary state and of the optimal cost functions then communicate them to the coordinator who in turn optimizes the boundary state to minimize the overall cost. By iterating between local operators and the coordinator, the proposed algorithm converges to the global optimal solution in finite steps, and it requires limited information sharing.

==> Application.tex <==
%application methods \subsection{System partition}
\indent Fluctuations of power flow distribution can be attributed as fluctuation of power injections. Hence in this paper, fluctuation sources are modeled as injections. For fluctuation source $i$, we know its connecting node $k_{i}$, standard error for fluctuation of active and reactive power injections $\Delta P_{i}$ and $\Delta Q_{i}$. The values for $\Delta P_{i}$ and $\Delta Q_{i}$ can be assigned by operation experience. Especially, for wind farms, these values can be set according to the variance of real-time wind power prediction. Subsequently, the fluctuation level of power flow on branch $l$, denoted by $\Delta P_{l}$ and $\Delta Q_{l}$, can be computed by:
\begin{equation}
\begin{array}{lll}
\Delta P_{l}&=&\sum \limits_{i=1}^{n}|S_{P}(k_{i},l)\Delta P_{i}|,\\
\Delta Q_{l}&=&\sum \limits_{i=1}^{n}|S_{Q}(k_{i},l)\Delta Q_{i}|.
\end{array}\label{eq:line_delta}
\end{equation}
where $S_{P}(k_{i},l)$ is the entry corresponding to node $k_{i}$ and branch $l$ in active power shift factor matrix, and $S_{Q}(k_{i},l)$ is the same entry in reactive power shift factor matrix. Scalar $n$ denotes the number of fluctuation sources.\\
\indent The fluctuation level of node $j$ is $\Delta_{j}$ defined by:
\begin{equation}
\begin{array}{lll}
\Delta P_{j}&=&\max \limits_{l\in \mathcal{A}_{j}}P_{l},\\
\Delta Q_{j}&=&\max \limits_{l\in \mathcal{A}_{j}}Q_{l},\\
\Delta_{j}&=&\sqrt{\Delta P_{j}^{2}+\Delta Q_{j}^{2}}.
\end{array}\label{eq:node_delta}
\end{equation}
where $\mathcal{A}_{j}$ denotes the adjacent branch set for node $j$.\\
\indent With the fluctuation level of each node, the system node set $\mathcal{N}$ is partitioned into steady area node set $\mathcal{N_{S}}$, quasi-steady area node set $\mathcal{N_{Q}}$ and fluctuant area node set $\mathcal{N_{F}}$:
\begin{equation}
\begin{array}{lll}
\mathcal{N_{S}}&=&\{j\in\mathcal{N}|\Delta_{j}\leq\epsilon_{q}\},\\
\mathcal{N_{Q}}&=&\{j\in\mathcal{N}|\epsilon_{q}<\Delta_{j}\leq\epsilon_{f}\},\\
\mathcal{N_{F}}&=&\{j\in\mathcal{N}|\Delta_{j}>\epsilon_{f}\}.
\end{array}\label{eq:sys_partition}
\end{equation}
where $\epsilon_{q}$ and $\epsilon_{f}$ are artificial thresholds.\\
\indent Similarly, the system measurement set $\mathcal{M}$ is also partitioned into steady area measurement set $\mathcal{M_{S}}$, quasi-steady area measurement set $\mathcal{M_{Q}}$ and fluctuant area measurement set $\mathcal{M_{F}}$. The steady area measurement set $\mathcal{M_{S}}$ includes measurements for node in $\mathcal{N_{S}}$ and measurements for head (tail) side for branches whose head (tail) nodes are in $\mathcal{N_{S}}$.\\
\indent Note that the system partition can change with system operations. Hence it is necessary to update the system partition after system operations are scheduled.
\subsection{State estimation method}
\indent Take steady area as example, its states are denoted by vector $x_{S}$, and the states for nodes outside but adjacent to steady area are denoted by $x_{BS}$. Then the measurement functions for steady area are:
\begin{equation}
z_{S}=h_{S}(x_{S},x_{BS})+e_{S}.\label{eq:meas_steadyarea}
\end{equation}
where $z_{S}$, $h_{S}$ and $e_{S}$ denote, respectively, measurement values, measurement functions and errors for measurement set $\mathcal{M_{S}}$.\\
\indent The state estimates for steady area are obtained by solving following weighted least square problem:
\begin{equation}
\begin{array}{ll}
\min \limits_{x_{S}}& (z_{S}-h_{S}(x_{S},x_{BS}))^{\dagger}W_{S}(z_{S}-h_{S}(x_{S},x_{BS})).
\end{array}\label{eq:semodel_steadyarea}
\end{equation}
where $W_{S}$ is the weight matrix for measurement set $\mathcal{M_{S}}$.
\indent Model (\ref{eq:semodel_steadyarea}) estimates the states in steady area with states in quasi-steady and fluctuant areas fixed. Similarly, the state estimation in quasi-steady and fluctuant areas will only update their own states as well. At any time moment $t$, the state estimates for the entire power system is given by:
\begin{equation}
\hat{x}=[\hat{x}_{S},\hat{x}_{Q},\hat{x}_{F}].\label{eq:se_fusion}
\end{equation}
where $\hat{x}_{S}$, $\hat{x}_{Q}$ and $\hat{x}_{F}$ are newest state estimates for steady area, quasi-steady area and fluctuant area, respectively.
\indent There are several effective hybrid PSSE methods, in this paper we use the method in \cite{Zhou_PWRS2006} for hybrid PSSE. The PSSE method with pure PMU measurements are given in section \ref{sec:concept}. 

==> LocalED.tex <==
%Local ED Part
%\subsection{Feasibility Check}\label{sec:FC}
%\indent In this subsection, a feasibility check method for the local ED in area $i$ is provided. The primal feasibility check model for the local ED in area $i$ is as follows:
%\begin{equation}
%\begin{array}{ll}
%\max \limits_{g_{i}}&0,\\
%\mbox{s.t.}&\hspace{0.25cm}M_{i}g_{i}+M_{B}\theta_{B}+M_{C}=0,\\
%\mbox{}&\hspace{0.25cm}N_{i}g_{i}+N_{B}\theta_{B}+N_{C}\leq 0.
%\end{array}\label{eq:13}
%\end{equation}
%\indent The dual problem of (\ref{eq:13}) is given by
%\begin{equation}\hspace{-0.1cm}
%\begin{array}{ll}
%\min\limits_{\lambda_i,\mu_{i}}&\hspace{-0.25cm}\omega(\lambda_i,\mu_{i})\hspace{-0.1cm}=\hspace{-0.1cm}-\lambda_i^{\dagger}(M_B\theta_B\hspace{-0.1cm}+\hspace{-0.1cm}M_C)\hspace{-0.1cm}-\hspace{-0.1cm}\mu_i^{\dagger}(N_B\theta_B\hspace{-0.1cm}+\hspace{-0.1cm}N_C),\\
%\mbox{s.t.}&\hspace{-0.25cm} \lambda^{\dagger}_{i}M_{i}+\mu_i^{\dagger}N_i=0,\mu_{i} \geq 0,
%\end{array}\label{eq:14}
%\end{equation}
%where $\lambda_{i}$ and $\mu_{i}$ denotes multipliers for equality and inequality constraints in (\ref{eq:13}), respectively. If $\omega^{*}<0$, the local ED in area $i$ is infeasible, and following inequalities can be given to guarantee the feasibility:
%\begin{equation}
%\begin{array}{l}
%E_B\theta_B+E_C\leq 0,\\
%E_B\hspace{-0.1cm}=\hspace{-0.1cm}(\lambda_i^*)^{\dagger}M_B\hspace{-0.1cm}+\hspace{-0.1cm}(\mu_i^*)^{\dagger}N_B, E_C\hspace{-0.1cm}=\hspace{-0.1cm}(\lambda_i^*)^{\dagger}M_C\hspace{-0.1cm}+\hspace{-0.1cm}(\mu_i^*)^{\dagger}N_C.
%\end{array}\hspace{-0.1cm}\label{eq:15}
%\end{equation}
%where $\lambda_i^*$ and $\mu^{*}_{i}$ is the solution to model (\ref{eq:14}). Considering numerical errors of local optimizers, in practical application, (\ref{eq:15}) needs to be slacked as
%\begin{equation}
%E_B\theta_B+E_C\leq\tau,\label{eq:15slack}
%\end{equation}
%where $\tau$ is a small negative constant.
\subsection{Critical Region Determination}\label{sec:CR}
\indent With given $\theta_B$, each area derives the explicit definition of current critical region containing the point of $\theta_B$ and the optimal cost function defined in current critical region.\\
\indent The Lagrange function for the local ED model (\ref{eq:local_MPQP}) is
\begin{equation}
\begin{array}{ll}
\!\!\!\!\!\!L(g_{i},\lambda_{i},\mu_{i})\!\!=\!\!&\!\!\!\!c_{i}\!+\!\lambda_{i}^{\dagger}(M_ig_{i}\!+\!M_B\theta_{B}\!+M_C)\\
\!\!\!\!&\!\!\!\!+\mu_{i}^{\dagger}(N_ig_i+N_B\theta_B+N_C).
\end{array}\label{eq:16}
\end{equation}
where $\lambda_{i}$ and $\mu_{i}$ denote multipliers for the equality and inequality constraints in the local ED model (\ref{eq:local_MPQP}), respectively. The KKT conditions for model (\ref{eq:local_MPQP}) are
\begin{eqnarray}
\!\!\left[\!\!\!\!
\begin{array}{ccc}
\setlength{\arraycolsep}{0.01pt}
2A_{i}\!\!\!\!&\!\!\!\!M_i^{\dagger}\!\!\!&\!\!\!\{N_i\}_{\mathcal{A}}^{\dagger}\\
M_i\!\!\!\!&\!\!\!\!\mbox{}\!\!\!&\!\!\!\mbox{}\\
\{N_i\}_{\mathcal{A}}\!\!\!\!&\!\!\!\!\mbox{}\!\!\!&\!\!\!\mbox{}
\end{array}
\!\!\!\!\right]\!\!\left[\!\!\!\!
\begin{array}{ccc}
g_{i}\\
\lambda_{i}\\
\{\mu_{i}\}_{\mathcal{A}}
\end{array}\!\!\!\!\right]
\!\!=\!\!\left[\!\!\!
\begin{array}{ccc}
-B_{i}\\
-M_B\theta_B-M_C\\
-\{N_{B}\theta_B\!\!+\!\!N_{C}\}_{\mathcal{A}}
\end{array}
\!\!\!\right]\!\!,
\label{eq:17}\\
\{\mu_{i}\}_{\mathcal{A}}\geq0,\{N_{i}g_{i}+N_{B}\theta_{B}+N_{C}\}_{\mathcal{A}}=0,\nonumber\\
\{\mu_{i}\}_{\mathcal{I}}=0,\{N_{i}g_{i}+N_{B}\theta_{B}+N_{C}\}_{\mathcal{I}}\leq0,\nonumber
\end{eqnarray}
where $\{\centerdot\}_{\mathcal{I}}$ denotes variables for inactive constraints.\\
\indent Assuming model (\ref{eq:local_MPQP}) is non-degenerate, then (\ref{eq:17}) can be solved by taking inverse to its coefficient matrix:
\begin{equation}
\left[\!\!
\begin{array}{ccc}
\setlength{\arraycolsep}{0.1pt}
g_{i}\\
\lambda_{i}\\
\{\mu_{i}\}_{\mathcal{A}}
\end{array}\!\!\right]\!\!\!=\!\!\!
\left[\!\!
\begin{array}{ccc}
\setlength{\arraycolsep}{0.1pt}
K_{11}\!\!&\!\!K_{12}\!\!&\!\!K_{13}\\
K_{12}^{\dagger}\!\!&\!\!K_{22}\!\!&\!\!K_{23}\\
K_{13}^{\dagger}\!\!&\!\!K_{23}^{\dagger}\!\!&\!\!K_{33}
\end{array}
\!\!\right]\!\!\!
\left[\!\!\!
\begin{array}{ccc}
-B_{i}\\
-M_B\theta_B-M_C\\
-\{N_{B}\theta_B\!\!+\!\!N_{C}\}_{\mathcal{A}}
\end{array}
\!\!\!\right]\!\!.\label{eq:18}
\end{equation}
\indent For active constraints, their multipliers $\{\mu_{i}\}_{A}$ are affine functions of $\theta_{B}$ and yield
\begin{equation}
\begin{array}{ll}
\{\mu_{i}\}_{A}=&\hspace{-0.25cm}-(K_{32}M_B+K_{33}\{N_B\}_{\mathcal{A}})\theta_{B}\\
&\hspace{-0.25cm}-(K_{31}B_i+K_{32}M_C+K_{33}\{N_C\}_{\mathcal{A}})\geq0.
\end{array}
\label{eq:21}
\end{equation}
\indent The optimizer $g^{*}_{i}$ is also an affine function of $\theta_{B}$ as
\begin{equation}
\begin{array}{l}
g^{*}_{i}=R_B\theta_B+R_C,\\
R_B=-K_{12}M_B-K_{13}\{N_{B}\}_{\mathcal{A}},\\
R_C=-K_{11}B_{i}-K_{12}M_C-K_{13}\{N_C\}_{\mathcal{A}}.
\end{array}
\label{eq:22}
\end{equation}
\indent Then for inactive constraints, their values yield
\begin{equation}\label{eq:23}
\begin{array}{l}
(\{N_i\}_{\mathcal{I}}R_B+\{N_B\}_{\mathcal{I}})\theta_B\hspace{-0.05cm}+\hspace{-0.05cm}\{N_i\}_{\mathcal{I}}R_C\hspace{-0.05cm}+\hspace{-0.05cm}\{N_C\}_{\mathcal{I}}\leq 0.
\end{array}
\end{equation}
\indent By combining (\ref{eq:21}) and (\ref{eq:23}), the explicit definition of the current critical region $CR_{i,k}$ in area $i$ is given by
\begin{equation}
\begin{array}{l}
CR_{i,k}=\{\theta_B|S_{i}\theta_{B}+T_{i}\leq0\},\\
S_{i}=\left[
\begin{array}{l}
K_{32}M_B+K_{33}\{N_B\}_{\mathcal{A}}\\
\{N_i\}_{\mathcal{I}}R_B+\{N_B\}_{\mathcal{I}}
\end{array}
\right],\vspace{0.1cm}\\T_i=\left[
\begin{array}{l}
K_{31}B_i+K_{32}M_C+K_{33}\{N_C\}_{\mathcal{A}}\\
\{N_i\}_{\mathcal{I}}R_C\hspace{-0.05cm}+\hspace{-0.05cm}\{N_C\}_{\mathcal{I}}
\end{array}
\right].
\end{array}
\label{eq:24}
\end{equation}
\indent Inequality (\ref{eq:21}) defines active constraints via their multipliers, and inequality (\ref{eq:23}) defines inactive constraints via their values. Their intersection (\ref{eq:24}) defines current partition of active and inactive constraints, which also defines current critical region. The critical region defined by (\ref{eq:24}) is a polyhedron, which is consistent with theorem 1. The redundant inequalities should be removed from (\ref{eq:24}), with method in \cite{INEQ}.\\
\subsection{Optimal Cost Function}
\indent Within current critical region defined by (\ref{eq:24}), the expression of optimal cost function $J_{i}^{*}(\theta_{B})$ can be got by substituting (\ref{eq:22}) to the cost function (\ref{eq:edi_cost}):
\begin{equation}
\begin{array}{l}
J_{i}^{*}(\theta_{B})\hspace{-0.1cm}=\hspace{-0.1cm}c_i(g_i^{*}(\theta_B))\hspace{-0.1cm}=\hspace{-0.1cm}(R_B\theta_B\hspace{-0.1cm}+\hspace{-0.1cm}R_C)^{\dagger}A_i(R_B\theta_B\hspace{-0.1cm}+\hspace{-0.1cm}R_C)\\
+B_i^{\dagger}(R_B\theta_B+R_C)=\theta_B^{\dagger}\tilde{A}_i\theta_B+\tilde{B}_i^{\dagger}\theta_B+\tilde{C}_i,\\
\tilde{A}_i=R_B^\dagger A_iR_B,\tilde{B}_i=2R_B^{\dagger}A_iR_C+R_B^{\dagger}B_i.
\end{array}
\label{eq:28}
\end{equation}
%\indent Note that the optimal cost function (\ref{eq:28}) is accurate as long as the active constraint set does not change, i.e., the point of boundary states remains in current critical region defined by (\ref{eq:24}).\\
%\indent With given boundary states $\theta_B$, each area first checks the feasibility of its local ED problem. If local ED is infeasible, sends the feasibility constraint (\ref{eq:15slack}) to the coordinator. If local ED is feasible, derives its optimal cost function (\ref{eq:28}) and corresponding critical region (\ref{eq:24}) then communicates them to the coordinator.
%\subsection{Degeneracy and Differentiability of Optimal Value Function}\label{sec:Property}
%\indent In previous subsection the optimal value function is derived within the same critical region. To make the strategy for the coordinator, we need to study properties of optimal value functions $J_{i}^{*}(P_{Bi})$ throughout its feasible region $\tilde{\Theta}_{i}$. Theorem 1 already guarantees the continuity and convexity, but it does not guarantee differentiability. The differentiability of the optimal value function actually relates to the degeneracy problem.\\
%\indent Since matrix $A\succ0$, the degeneracy of model (\ref{eq:7}) is always caused by linear dependent active constraints. When model (\ref{eq:7}) is degenerate with given $P_{Bi}$, the optimal solution of $P_{i}$ is still unique, while multipliers may have infinite number of solutions. Review the derivative of the optimal value function with respect to interchange power $P_{Bi}$ in (\ref{eq:27}), the non-uniqueness of the multipliers may make the optimal value function non-differentiable.\\
%\indent To get rid of this problem, all inequality constraints in area $i$ are sorted in a certain sequence before coordinated ED computation. When model (\ref{eq:7}) is degenerate, i.e., the coefficient matrix in (\ref{eq:17}) is singular, assuming the rank of the coefficient matrix is $r$, then only the first $r-g_{i}-1$ linear independent constraints in the pre-determined sequence are set as active and the multipliers for the other inequality constraints are set as zero. Accordingly, whenever model (\ref{eq:7}) is degenerate, we can get unique solution of multipliers and the optimal value function will be differentiable. On the other hand, rows and columns correspond to constraints with zero multipliers should be removed in (\ref{eq:17}) and the rest coefficient matrix is full rank, then we can define current critical region (\ref{eq:24}) and derive the optimal value function (\ref{eq:28}) just like non-degenerate cases.\\
%\indent Now we consider the differentiability of the optimal value function, and following theorem can be proved:
%\begin{theorem}\label{theorem:continuity}
%With the dispose strategy of degeneracy described above, multipliers $\lambda_{i}$ and $\mu_{i}$ are continuous with respect to $P_{Bi}$ throughout the feasible region $\tilde{\Theta}_{i}$.
%\end{theorem}
%$Proof$: Inside each critical region, multipliers are affine functions of $P_{Bi}$ as (\ref{eq:18}) and always continuous. Hence the proof will focus on the boundary between different critical regions.\\
%\indent Without loss of generality, the boundary between critical regions $CR_{i,k1}$ and $CR_{i,k2}$, denoted by $\Lambda_{k1,k2}$, is considered. These two critical regions have different optimal partitions for constraints. Hence all inequality constraints can be divided into four subsets: constraints that are active in both critical regions, denoted by subscript $AA$; active in $CR_{i,k1}$ but inactive in $CR_{i,k2}$, denoted by subscript $AI$; inactive in $CR_{i,k1}$ but active in $CR_{i,k2}$, denoted by subscript $IA$; and inactive in both critical regions, denoted by subscript $II$. Note that when degeneracy happens, the redundant constraints are subsumed into inactive constraint set.\\
%\indent We first consider multiplier $\{\mu_{i}\}_{AI}$, the critical region $CR_{i,k1}$ is defined by
%\begin{equation}
%\begin{array}{l}
%\{\mu_{i}\}_{AI,AA}=\{W_{i}\}_{AI,AA}P_{Bi}+\{R_{i}\}_{AI,AA}\geq0,\\
%\{h_{i}\}_{IA,II}=\{W_{i}\}_{IA,II}P_{Bi}+\{R_{i}\}_{IA,II}\leq0.
%\end{array}\label{eq:CR1}
%\end{equation}
%\indent Critical region $CR_{i,k1}$ is a polyhedron and its boundary with $CR_{i,k2}$ can be expressed as\\
%\begin{equation}
%\begin{array}{lll}
%\Lambda_{k1,k2}&=\{P_{Bi}\in\tilde{\Theta}_{i}|\!&\{\mu_{i}\}_{AI}=0,\{\mu_{i}\}_{AA}>0,\\
%&&\{h_{i}\}_{IA}=0,\{h_{i}\}_{II}<0\}.
%\end{array}
%\label{eq:boundary}
%\end{equation}
%\indent And when the point of $P_{Bi}$ converges to $\Lambda_{k1,k2}$ in $CR_{i,k1}$, there is
%\begin{equation}
%\lim_{\substack{P_{Bi}\rightarrow\Lambda_{k1,k2}\\P_{Bi}\in CR_{i,k1}}}\{\mu_{i}\}_{AI}=0.\label{eq:muai}
%\end{equation}
%Note that in critical region $CR_{i,k2}$, there is $\{\mu_{i}\}_{AI}=0$. Hence $\{\mu_{i}\}_{AI}$ is continuous on the boundary $\Lambda_{k1,k2}$. Similarly, the multiplier $\{\mu_{i}\}_{IA}$ is also continuous.\\
%\indent Now we consider multipliers $\{\mu_{i}\}_{AA}$ and $\lambda_{i}$. In $CR_{i,k1}$, the KKT conditions are given by
%\begin{eqnarray}
%\left[
%\begin{array}{cccc}
%\setlength{\arraycolsep}{0.01pt}
%2A_{i}&1_{g_{i},1}&\{M_{ii}\}_{AA}^{\dagger}&\{M_{ii}\}_{AI}^{\dagger}\\
%1_{1,g_{i}}&\mbox{}&\mbox{}&\mbox{}\\
%\{M_{ii}\}_{AA}&\mbox{}&\mbox{}&\mbox{}\\
%\{M_{ii}\}_{AI}&\mbox{}&\mbox{}&\mbox{}
%\end{array}
%\right]\nonumber\\
%\left[
%\begin{array}{c}
%P_{i}\\
%\lambda_{i}\\
%\{\mu_{i}\}_{AA}\\
%\{\mu_{i}\}_{AI}
%\end{array}\right]=\left[
%\begin{array}{c}
%-B_{i}\\
%1_{1,d_{i}}D_{i}-1_{1,b_{i}}P_{Bi}\\
%\{N_{i}-M_{iB}P_{Bi}\}_{AA}\\
%\{N_{i}-M_{iB}P_{Bi}\}_{AI}
%\end{array}
%\right].
%\label{eq:30}
%\end{eqnarray}
%\indent Note that on the boundary $\Lambda_{k1,k2}$, there is $\{\mu_{i}\}_{AI}=0$, and the first three rows of (\ref{eq:30}) forms following equation
%\begin{equation}
%\!\left[\!\!\!\!
%\begin{array}{ccc}
%\setlength{\arraycolsep}{0.01pt}
%2A_{i}\!\!&\!\!1_{g_{i},1}\!\!&\!\!\{M_{ii}\}_{AA}^{\dagger}\\
%1_{1,g_{i}}\!\!&\!\!\mbox{}\!\!&\!\!\mbox{}\\
%\{M_{ii}\}_{AA}\!\!&\!\!\mbox{}\!\!&\!\!\mbox{}
%\end{array}
%\!\!\!\!\right]\!\!\!\!
%\left[\!\!\!\!
%\begin{array}{c}
%P_{i}\\
%\lambda_{i}\\
%\{\mu_{i}\}_{AA}
%\end{array}\!\!\!\!\right]\!\!\!=\!\!\!\left[\!\!\!\!
%\begin{array}{c}
%-B_{i}\\
%1_{1,d_{i}}D_{i}\!-\!1_{1,b_{i}}P_{Bi}\\
%\{N_{i}\!-\!M_{iB}P_{Bi}\}_{AA}
%\end{array}\!\!\!\!
%\right]\!\!.
%\label{eq:31}
%\end{equation}
%\indent Similarly, in  $CR_{i,k2}$, when $P_{Bi}\rightarrow\Lambda_{k1,k2}$, there is $\{\mu_{i}\}_{IA}\rightarrow0$, and the first three rows of its KKT conditions also form (\ref{eq:31}). Hence we have
%\begin{eqnarray}
%\lim_{\substack{P_{Bi}\rightarrow\Lambda_{k1,k2}\\P_{Bi}\in CR_{i,k1}}}\{\mu_{i}\}_{AA}&=&\lim_{\substack{P_{Bi}\rightarrow\Lambda_{k1,k2}\\P_{Bi}\in CR_{i,k2}}}\{\mu_{i}\}_{AA}\nonumber\\
%\lim_{\substack{P_{Bi}\rightarrow\Lambda_{k1,k2}\\P_{Bi}\in CR_{i,k1}}}\lambda_{i}&=&\lim_{\substack{P_{Bi}\rightarrow\Lambda_{k1,k2}\\P_{Bi}\in CR_{i,k2}}}\lambda_{i}
%\label{eq:32}
%\end{eqnarray}
%\indent Equation (\ref{eq:32}) proves the continuity of $\{\mu_{i}\}_{AA}$ and $\lambda_{i}$. Multipliers $\{\mu_{i}\}_{II}$ equal to zero in both critical regions. Hence in summary, the multipliers  $\lambda_{i}$ and $\mu_{i}$ are continuous throughout the feasible region $\tilde{\Theta}_{i}$. \QEDB \\
%\indent According to theorem \ref{theorem:continuity} and (\ref{eq:27}), following theorem can be proved:
%\begin{theorem}\label{theorem:differentiable}
%With the dispose strategy of degeneracy described above, the optimal value function $J_{i}^{*}(P_{Bi})$ is differentiable with respect to $\!P_{Bi}\!$ throughout the feasible region $\tilde{\Theta}_{i}$.
%\end{theorem}
%\par\indent The proof of theorem \ref{theorem:differentiable} can be got according to the expression of the gradient of $J_{i}^{*}(P_{Bi})$ in (\ref{eq:27}).\\
%\indent Hence in summary, the optimal value function $J_{i}^{*}(P_{Bi})$ is continuous, differentiable, convex, and piecewise quadratic throughout the feasible region $\tilde{\Theta}_{i}$. As the summation of optimal value functions in all areas, the objective function of the coordinator inherits all these properties. And it can be concluded that the coordinator model (\ref{eq:11}) is a convex programming problem with unique global optimum point. 

==> MPP.tex <==
%Preliminaries: introduce the basic concept of multi-parametric programming
The concept of critical region is related to multi-parametric programming. In this section, we briefly introduce some key concepts and results of multi-parametric quadratic program (MPQP). See \cite{MPP_QPLP} for a more detailed coverage.

MPQP with optimizers $x$ and parameters $\theta$ is defined by
\begin{equation}
\begin{array}{ll}
\min \limits_{x}&f(x)=x^{\dagger}Ax+B^{\dagger}x+C,\\
\mbox{s.t.}& h(x,\theta)=M_{x}x+M_{\theta}\theta -M_{c}\leq 0,\\
&\theta\in \Theta,\label{eq:pre1}
\end{array}
\end{equation}
where matrix $A$, vector $B$, and scalar $C$ are coefficients of the quadratic objective function, and $M_{x}$, $M_{\theta}$, and $M_{c}$ are coefficients of linear constraints. The superscript $\dagger$ denotes transpose. In this paper, we consider matrix $A\succ0$, and if the MPQP (\ref{eq:pre1}) is feasible, it has unique optimal solution.

In MPQP, we derive the optimizer and optimal value as functions of parameters, denoted by $x^{*}(\theta)$ and $J^{*}(\theta)=f(x^{*}(\theta))$, respectively. The KKT conditions for problem (\ref{eq:pre1}) are given by
\begin{equation}
\nabla_{x}f+\{\mu^{\dagger}M_{x}\}_{\mathcal{A}}=0, \{M_{x}x+M_{\theta}\theta -M_{c}\}_{\mathcal{A}}=0,\mu\geq0,
\label{eq:prekkt}
\end{equation}
where $\{\centerdot\}_{\mathcal{A}}$ denotes variables associated with active constraints. The solution of (\ref{eq:prekkt}) gives the expression of the optimizer $x^{*}(\theta)$, which turns out to be an affine function of parameters $\theta$:
\begin{equation}
x^{*}(\theta)=K\theta+Q.
\label{eq:preoptimzer}
\end{equation}
\indent Accordingly, the critical region is defined as the set of parameters for which the optimizer computed by (\ref{eq:preoptimzer}) remains optimal.

For the MPQP, we have the following theorem \cite{MPP_QPLP}:

\textit{\textbf{Theorem}} 1: Consider the multi-parametric quadratic programming (\ref{eq:pre1}), assuming the region $\Theta$ is convex. Then

i) $x^{*}(\theta)$ is continuous and piecewise affine in $\Theta$;

ii) Optimal value function $J^{*}(\theta)$ is continuous, convex, and piecewise quadratic in $\Theta$.

\indent Note that on the boundary of critical regions, some constraints, denoted by subscript $\mathcal{C}$, yield to
\begin{equation}
\{M_{x}x+M_{\theta}\theta -M_{c}\}_{\mathcal{C}}=0, \{\mu\}_{\mathcal{C}}=0.\label{eq:precri}
\end{equation}
In this paper, such constraints are also referred to as critical constraints. For any constraint, when its status switches between inactive or active and critical, KKT conditions will not change. Therefore, the optimality for (\ref{eq:preoptimzer}) remains on the boundary of critical regions and critical regions are defined as closed sets.\footnote{Some other literature define critical regions as open or half-open-half-closed sets. Minor changes to the proposed method are needed if a different definition to critical region is used. Without loss of generality, we follow in this paper the definition in \cite{MPP_QPLP}.}

Generally, the solution of MPQP gives the optimal value functions in all critical regions, which can be computationally costly. In this paper, however, we do not really solve the MPQP problem, but only determine the current critical region to which the given $\theta$ belongs. 

==> Theoretical.tex <==
%Theoretical
\indent In this section we will study the convergence of the proposed coordinated economic dispatch method. There are two optimization problems in coordinated dispatch: local ED and coordinator optimization. The local ED is a convex quadratic programming problem and its convergence is robust. Hence our major concern is the convergence of the coordinator, which objective function and constraints will change in different critical regions.\\
\indent For the coordinator model (\ref{eq:37}), assume its global optimum point is $P_{ij}^{*}$, then the line segment between $P_{ij}^{*}$ and any given point $P_{ij}$ is denoted by $\Lambda(P_{B})$:
\begin{equation}
\Lambda(P_{B})=\{y\in \tilde{\Theta}|y=\alpha P_{B}^{*}+(1-\alpha)P_{B}, 0<\alpha<1\}
\label{eq:cvg1}
\end{equation}
\indent Then following lemmas can be proved:
\begin{lemma}
The objective function $J_{\Sigma}(y(\alpha))$ is a monotonic decrease function with respect to $\alpha$.
\label{lemma:2}
\end{lemma}
 $Proof$: According to the convexity of theorem 2, for any $0\leq\alpha_{1}<\alpha_{2}\leq1$,we have:
 \begin{equation}
J_{\Sigma}(y(\alpha_{1}))\!-\!J_{\Sigma}(y(\alpha_{2}))\!>\!\nabla_{P_{ij}}J_{\Sigma}(y(\alpha_{2}))^{T}(y(\alpha_{1})\!-\!y(\alpha_{2})).\label{eq:cvg2}
\end{equation}
\indent Note that points $P_{ij}^{*}$, $y(\alpha_{1})$ and $y(\alpha_{2})$ lie on the same line segment and $P_{ij}^{*}$ is the optimum point, hence the right hand side in (\ref{eq:cvg2}) is positive. And we can have $J_{\Sigma}(y(\alpha_{1}))-J_{\Sigma}(y(\alpha_{2}))>0$, which proves lemma \ref{lemma:2}.  \QEDB
\indent With lemma \ref{lemma:2}, we can have following lemma:
\begin{lemma}
In iteration $t$, assume that:\\
1) We have point $P_{ij}^{(t)}$ and critical region $\Theta^{(t)}$;\\
2) The optimum point $P_{ij}^{*}$ does not lie in $\Theta^{(t)}$.\\
Then the line segment $P_{ij}^{(t+1)}-P_{ij}^{*}$ has no point inside $\Theta^{(t)}$.
\label{lemma:3}
\end{lemma}
$Proof$: By contradiction, assume there exists $y(\alpha)=\alpha P_{ij}^{*}+(1-\alpha)P_{ij}^{(t+1)}, 0<\alpha<1$ and $y(\alpha)\in\Theta^{(t)}$. According to lemma \ref{lemma:2}, we have $J_{\Sigma}(y)<J_{\Sigma}(P_{ij}^{(t+1)})$. Furthermore, as point $y\in\Theta^{(t)}$, the coordination in iteration $t$ should not converge to $P_{ij}^{(t+1)}$. Hence in summary, our assumption cannot hold and the line segment $P_{ij}^{(t+1)}-P_{ij}^{*}$ has no point inside $\Theta^{(t)}$. \QEDB \\
\indent With these two lemmas, we can illustrate how our hierarchical ED converges to the optimum point. Take Fig.\ref{fig:3}(c) as example, there are six critical regions for the overall ED problem. Since the overall ED inside each critical region is a convex programming problem, there is an unique optimum point for each critical region. Assume the optimum point $P_{ij}^{*}$ lies in $\bar{\Theta_{3}}$, then the optimum point in $\bar{\Theta_{3}}$ is $P_{ij,3}^{*}=P_{ij}^{*}$. The other critical regions have no stationary point and their optimum points will lie on the boundaries, as shown in Fig.\ref{fig:3}(c). Assume the initial point $P_{ij}^{0}$ lies in $\Theta_{1}$, then in the first iteration, the coordinator will search an optimum point in $\bar{\Theta_{1}}$ and it will get  $P_{ij,1}^{*}$. In the second iteration, the optimization enters $\bar{\Theta_{2}}$ and the coordinator will get $P_{ij,2}^{*}$. And in the third iteration, the optimization enters $\bar{\Theta_{3}}$ and the coordinator will finally converge to $P_{ij}^{*}$. Note that for a given overall ED problem, the partition of critical regions and the optimum point in each critical region are fixed. Hence there are certain tracks that composed by the point sequence of optimum point in each area and converge to $P_{ij}^{*}$. Take Fig.\ref{fig:3}(c) as example, there are two tracks($P_{ij,1}^{*}\rightarrow P_{ij,2}^{*}\rightarrow P_{ij}^{*}$ and $P_{ij,4}^{*}\rightarrow P_{ij,5}^{*}\rightarrow P_{ij,6}^{*}\rightarrow P_{ij}^{*}$). For any initial point $P_{ij}^{0}$, it will move to the optimum point of its critical region in the first iteration, then consequent iterations will converge to $P_{ij}^{*}$ along one of these certain tracks. Hence we have following theorem concerning the convergence speed of hierarchical ED:
\begin{theorem}
Assume that the initial point $P_{ij}^{0}\in\Theta_{k}$, then the hierarchical ED method needs $v_{k}+1$ iterations to converge to the final optimum point $P_{ij}^{*}$. $v_{k}$ is the difference between the indices of  $P_{ij,k}^{*}$ and $P_{ij}^{*}$ in the point sequence defined by the track that contains $P_{ij,k}^{*}$.
\label{theorem:convergence}
\end{theorem}
\indent Theorem \ref{theorem:convergence} guarantees that hierarchical ED can converge at any cases with limited iterations.


